Diversifying Dialogue Generation with Non-Conversational Text

Neural network-based sequence-to-sequence (seq2seq) models strongly suffer from the low-diversity problem when it comes to open-domain dialogue generation. As bland and generic utterances usually dominate the frequency distribution in our daily chitchat, avoiding them to generate more interesting responses requires complex data filtering, sampling techniques or modifying the training objective. In this paper, we propose a new perspective to diversify dialogue generation by leveraging non-conversational text. Compared with bilateral conversations, non-conversational text are easier to obtain, more diverse and cover a much broader range of topics. We collect a large-scale non-conversational corpus from multi sources including forum comments, idioms and book snippets. We further present a training paradigm to effectively incorporate these text via iterative back translation. The resulting model is tested on two conversational datasets and is shown to produce significantly more diverse responses without sacrificing the relevance with context.

==> model_fig.tex <==
\tikzset{
  emb/.style = {draw, rectangle, fill=cosmos, minimum width=3em, minimum height=1.3em, inner sep=0, outer sep=0},
  transformer/.style = {draw, rectangle, fill=cruise, minimum width=3em, minimum height=1.5em},
  norm/.style = {draw, rectangle, fill=spring_sun, minimum width=4.5em, minimum height=1em, inner sep=0, outer sep=0},
  dropout/.style = {draw, rectangle, fill=hint_green, minimum width=4.5em, minimum height=1em, inner sep=0, outer sep=0},
  mh/.style = {draw, rectangle, fill=dairy_cream, minimum width=4.5em, minimum height=1.5em},
  ff/.style = {draw, rectangle, fill=french_pass, minimum width=4.5em, minimum height=1.5em},
  posemb/.style = {draw, rectangle, fill=watusi, minimum width=3em, minimum height=1.3em, inner sep=0, outer sep=0},
  proj/.style = {draw, rectangle, fill=Madang, minimum width=3em, minimum height=1.5em, inner sep=0, outer sep=0},
  FARROW/.style={arrows={-{Latex[length=1mm, width=0.8mm]}}}
}

\begin{figure*}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tikzpicture}

\node[emb] (e1) at (0, 0) {$\bm{v}_1$};
\node[right of=e1, node distance=1.2cm] (e2) {$\cdots$};
\node[emb, right of=e2, node distance=1.2cm] (e3) {$\bm{v}_{t-1}$};
\node[emb, right of=e3, node distance=2cm] (e4) {$\bm{v}_{\scaleto{\text{[mask]}}{3pt}}$};

\node[below of=e1, node distance=1.5cm] (i1) {$v_1$};
\node[below of=e2, node distance=1.5cm] (i2) {$\cdots$};
\node[below of=e4, node distance=1.5cm] (i4) {\small{[mask]}};
\node[below of=e3, node distance=1.5cm] (i3) {$v_{t-1}$};

\foreach \x in {1,3,4}
{
\node[transformer, above of=e\x, node distance=1.2cm] (t\x) {Trm};
\node[above of=t\x, node distance=1cm] (d\x) {$\vdots$};
\node[transformer, above of=d\x, node distance=1cm] (tt\x) {Trm};
\node[below of=e\x, node distance=0.4cm] (add\x) {\huge\textbf{+}};
}

\draw [decorate, decoration={brace,amplitude=5pt}] ([xshift=-1mm] t1.south west) -- ([xshift=-1mm] tt1.north west) node[midway,xshift=-0.4cm, align=center] (w) {$L\times$};
    
    
\node[posemb, below of=e1, node distance=0.8cm] (pe1) {$\bm{p}_1$};
\node[below of=e2, node distance=0.8cm] (pe2) {$\cdots$};
\node[posemb, below of=e3, node distance=0.8cm] (pe3) {$\bm{p}_{t-1}$};
\node[posemb, below of=e4, node distance=0.8cm] (pe4) {$\bm{p}_{t}$};

\node[proj, above of=tt4, node distance=0.95cm] (proj1) {\scriptsize Projection};

\node[above of=tt1, node distance=0.8cm] (o1) {};
\node[above of=tt1, node distance=0.55cm, xshift=0.23cm] (oa1) {\scriptsize$\bm{h}_1^L$};
\node[above of=tt3, node distance=0.8cm] (o3) {};
\node[above of=tt3, node distance=0.55cm, xshift=0.35cm] (oa3) {\scriptsize$\bm{h}_{t-1}^L$};
\node[above of=proj1, node distance=0.8cm] (o4) {$v_{t}$};
\node[above of=tt4, node distance=0.55cm, xshift=0.25cm] (oa4) {\scriptsize$\bm{h}_{t}^L$};

\draw[FARROW] (tt4) -> (proj1) ;
\draw[FARROW] (proj1) -> (o4) ;
\draw[FARROW] (tt1) -> (o1) ;
\draw[FARROW] (tt3) -> (o3) ;


\draw[FARROW] (i1.east) -- ++(0.45, 0) |-  (e1.east) ;
\draw[FARROW] (i3.east) -- ++(0.3, 0) |-  (e3.east) ;
\draw[FARROW] (i4.east) -- ++(0.2, 0) |-  (e4.east) ;

\foreach \x in {1,3,4}
{
\draw[FARROW] (i\x) -- (pe\x) ;
}

\draw [decorate, decoration={brace,amplitude=5pt}] ([xshift=-1mm] pe1.south west) -- ([xshift=-1mm] e1.north west) node[midway,xshift=-0.5cm, rotate=90, align=center, font=\scriptsize] (w) {Embedding\\ Layer};

\foreach \x in {1,3,4}
{
\foreach \y in {1,3,4}
{
    \draw[FARROW] (e\x.north) -> (t\y.south) ;
    \draw[FARROW] (t\x.north) -> (d\y.south) ;
    \draw[FARROW] ($(d\x.north)+(0, -0.15)$) -> (tt\y.south) ;
}
}
\node[above of=e2, node distance=1.2cm] (t2) {$\cdots$};
\node[above of=t2, node distance=1cm] (d2) {$\vdots$};
\node[above of=d2, node distance=1cm] (tt2) {$\cdots$};

 

\node[mh, left of=e1, node distance=3.2cm, align=center, font=\scriptsize, yshift=-0.3cm] (trm1) {Multi-Head\\ Attention};
\node[dropout, above of=trm1, node distance=0.75cm, align=center, font=\scriptsize] (do1) {Dropout};
\node[norm, above of=do1, node distance=0.6cm, align=center, font=\scriptsize] (n1) {Add \& Norm};

\draw[FARROW] (trm1) edge (do1);
\draw[FARROW] (do1) edge (n1);

\node[ff, above of=n1, node distance=1cm, align=center, font=\scriptsize] (ff1) {Position-wise\\Feed-Forward};
\node[dropout, above of=ff1, node distance=0.75cm, align=center, font=\scriptsize] (do2) {Dropout};
\node[norm, above of=do2, node distance=0.6cm, align=center, font=\scriptsize] (n2) {Add \& Norm};

\draw[FARROW] (n1) edge (ff1);
\draw[FARROW] (ff1) edge (do2);
\draw[FARROW] (do2) edge (n2);

\node[below of=trm1, node distance=1.2cm, align=center, font=\small] (input) {input};
\node[above of=n2, node distance=0.8cm, align=center, font=\scriptsize] (out) {};
\node[right of=out, node distance=0.7cm, align=center, font=\scriptsize, yshift=-0.35cm] (aa) {Trm};


\draw[FARROW] (n2) edge (out);
\draw[FARROW] (input) edge (trm1);

\draw[FARROW] ($(input.north)-(0,-0.3)$) -- ++(-1, 0) |- (n1.west) ;
\draw[FARROW] ($(n1.north)-(0,-0.3)$) -- ++(-1, 0) |- (n2.west) ;

\draw[thick,dotted, fill opacity=0.1, fill=bgc]  ($(input.south west)+(-0.8, 0.6)$) rectangle ($(out.north east)+(0.8, -0.6)$);

    

\node[below of=i2, node distance=0.6cm, xshift=1cm] (bert) {(b) BERT4Rec model architecture.};
\node[left of=bert, node distance=5.4cm] (trm) {(a) Transformer Layer.};

\node[emb, right of=e4, node distance=3cm, yshift=-0.8cm, minimum height=1.2em] (u1) {};

\node[right of=u1, node distance=1.2cm, minimum height=1.2em] (u2) {$\cdots$};
\node[emb, right of=u2, node distance=1.2cm, minimum height=1.2em] (u3) {};
\node[emb, right of=u3, node distance=2cm, minimum height=1.2em] (u4) {};

\node[below of=u1, node distance=0.7cm] (ui1) {$v_1$};
\node[below of=u2, node distance=0.7cm] (ui2) {$\ldots$};
\node[below of=u4, node distance=0.7cm] (ui4) {$v_{t}$};
\node[below of=u3, node distance=0.7cm] (ui3) {$v_{t-1}$};

\foreach \x in {1,3,4}
{
\node[transformer, above of=u\x, node distance=0.8cm, minimum height=1.2em, inner sep=0, outer sep=0] (ut\x) {GRU};
\draw[FARROW] (u\x) edge (ut\x) ;
}
\node[above of=u2, node distance=0.8cm] (ut2) {$\ldots$};
\foreach \x/\y in {1/2, 2/3, 3/4}
{
\draw[FARROW] (ut\x) edge (ut\y) ;
}

\node[above of=ut1, node distance=0.7cm] (utt1) {$v_2$};
\node[above of=ut2, node distance=0.7cm] (utt2) {$\ldots$};
\node[above of=ut3, node distance=0.7cm] (utt3) {$v_{t}$};
\node[above of=ut4, node distance=0.7cm] (utt4) {$v_{t+1}$};
\foreach \x/\y in {1,3,4}
{
\draw[FARROW] ($(ui\x.north)-(0,0.08)$) -> (u\x) ;
\draw[FARROW] (ut\x) -> ($(utt\x.south)-(0,-0.08)$) ;
}

\draw[thick,dotted]  ($(ui1.south west)+(-0.4, 0)$) rectangle ($(utt4.north east)+(0.4, 0)$);
\node[below of=ui2, node distance=0.6cm, xshift=1.1cm] (rnn) {(d) RNN based sequential recommendation methods.};

\foreach \x in {1,3,4}
{
\node[emb, above of=utt\x, node distance=2cm, minimum height=1.2em] (sa\x) {};
\node[transformer, above of=sa\x, node distance=0.8cm, minimum height=1.2em, inner sep=0, outer sep=0] (st\x) {Trm};
\node[transformer, above of=st\x, node distance=0.8cm, minimum height=1.2em, inner sep=0, outer sep=0] (stt\x) {Trm};
}
\node[below of=sa1, node distance=0.7cm] (si1) {$v_1$};
\node[below of=sa3, node distance=0.7cm] (si3) {$v_{t-1}$};
\node[below of=sa4, node distance=0.7cm] (si4) {$v_{t}$};
\node[right of=sa1, node distance=1.2cm, minimum height=1.2em] (sa2) {$\ldots$};

\node[below of=sa2, node distance=0.7cm, minimum height=1.2em] (si2) {$\ldots$};
\node[above of=sa2, node distance=0.8cm, minimum height=1.2em] (st2) {$\ldots$};
\node[above of=st2, node distance=0.8cm, minimum height=1.2em] (stt2) {$\ldots$};
\node[above of=stt1, node distance=0.7cm] (so1) {$v_2$};
\node[above of=stt3, node distance=0.7cm] (so3) {$v_{t}$};
\node[above of=stt4, node distance=0.7cm] (so4) {$v_{t+1}$};

\foreach \x in {1,3,4}
{
\draw[FARROW] ($(si\x.north)-(0,0.08)$) -> (sa\x) ;
\draw[FARROW] (sa\x.north) -> (st\x.south) ;
\draw[FARROW] (st\x.north) -> (stt\x.south) ;
\draw[FARROW] (stt\x) -> ($(so\x.south)-(0,-0.08)$) ;
}

\foreach \x/\y in {1/3, 1/4, 3/4}
{
\draw[FARROW] (sa\x.north) -> (st\y.south) ;
\draw[FARROW] (st\x.north) -> (stt\y.south) ;
}

\draw[thick,dotted]  ($(si1.south west)+(-0.4, 0)$) rectangle ($(so4.north east)+(0.4, 0)$);
\node[below of=si2, node distance=0.6cm, xshift=1cm] (sas) {(c) SASRec model architecture.};

\end{tikzpicture}}
    \caption{Differences in sequential recommendation model architectures. BERT4Rec learns a bidirectional model via Cloze task, while SASRec and RNN based methods are all left-to-right unidirectional model which predict next item sequentially.}
    \label{fig:model}
\end{figure*}



\tikzset{
  emb/.style = {draw, rectangle, fill=cosmos, minimum width=3em, minimum height=1.3em, inner sep=0, outer sep=0},
%   Seq2seq/.style = {draw, rectangle, fill=hint_green, minimum width=5em, minimum height=1.3em},
  Seq2seq/.style = {draw, rectangle, fill=cruise, minimum width=8em, minimum height=1.7em},
  transformer/.style = {draw, rectangle, fill=cruise, minimum width=3em, minimum height=1.5em},
  norm/.style = {draw, rectangle, fill=spring_sun, minimum width=4.5em, minimum height=1em, inner sep=0, outer sep=0},
  dropout/.style = {draw, rectangle, fill=hint_green, minimum width=4.5em, minimum height=1em, inner sep=0, outer sep=0},
  mh/.style = {draw, rectangle, fill=dairy_cream, minimum width=4.5em, minimum height=1.5em},
  ff/.style = {draw, rectangle, fill=french_pass, minimum width=4.5em, minimum height=1.5em},
  posemb/.style = {draw, rectangle, fill=watusi, minimum width=3em, minimum height=1.3em, inner sep=0, outer sep=0},
  proj/.style = {draw, rectangle, fill=Madang, minimum width=3em, minimum height=1.3em, inner sep=0, outer sep=0},
  FARROW/.style={arrows={-{Latex[length=1mm, width=0.8mm]}}}
}

\begin{figure*}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tikzpicture}

\node[emb] (e1) at (0, 0) {$D_{X'}$};
\node[emb, right of=e1, node distance=1.2cm] (e2) {$D_{T'}$};
\node[Seq2seq, above of=e1, node distance=0.8cm, minimum height=1.2em] (se2) {$S2S_{D_{X}->D_{Y}}+LM(D_{T})$};
\node[posemb, above of=se2, node distance=0.8cm] (pe1) {$Gen\;R$};
\node[proj, above of=pe1, node distance=0.8cm] (pe2) {$LM_{(D_{Y})}$};

% \node[emb] (e1) at (0, 0) {$\bm{v}_1$};
% \node[right of=e1, node distance=1.2cm] (e2) {$\cdots$};

\end{tikzpicture}}
    \caption{Differences in sequential recommendation model architectures. BERT4Rec learns a bidirectional model via Cloze task, while SASRec and RNN based methods are all left-to-right unidirectional model which predict next item sequentially.}
    \label{fig:model2}
\end{figure*}

